FMI: Fast and Cheap Message Passing for Serverless Functions

Serverless functions provide elastic scaling and a fine-grained billing model, making Function-as-a-Service (FaaS) an attractive programming model. However, for distributed jobs that benefit from large-scale and dynamic parallelism, the lack of fast and cheap communication is a major limitation. We overcome this limitation and present the FaaS Message Interface (FMI). FMI is an easy-to-use, high-performance framework for general-purpose point-to-point and collective communication in FaaS applications. We support different communication channels and offer a model-driven channel selection according to performance and cost expectations. We model the interface after MPI and show that message passing can be integrated into serverless applications with minor changes, providing portable communication closer to that offered by high-performance systems. In our experiments, FMI can speed up communication for a distributed machine learning FaaS application by up to 162x, while simultaneously reducing cost by up to 397 times.

==> latex-tools-overleaf/config.tex <==

\usepackage{etoolbox}

\newtoggle{AlgsNoEnd}


==> latex-tools-overleaf/includes.tex <==


\newif\iftr     % Full arXiv technical report
\newif\ifconf   % Size-constrainted Submission to a conf or journal
\newif\ifnonb   % Non blind submission

%%%%%%%%%%%%%
% Various
%%%%%%%%%%%%%
\usepackage[utf8]{inputenc}
\newcommand{\code}[1]{\texttt{#1}}
% binary units
\usepackage[binary-units=true]{siunitx}
\usepackage{xspace}
\usepackage[svgnames]{xcolor}

%%%%%%%%%%%%%
% Notes
%%%%%%%%%%%%%
\usepackage{collab}
% Define author:
%\collabAuthor{cmd_name}{color}{display_name}

%%%%%%%%%%%%%
% Bibliography
%%%%%%%%%%%%%
% citep
\usepackage[numbers,sort&compress]{natbib}

%%%%%%%%%%%%%
% Highlight
%%%%%%%%%%%%%
\usepackage{soul}
\soulregister\cite7
\soulregister\autoref7
\soulregister\code7
\soulregister\toolname7
\soulregister\ref7
\soulregister\pageref7
\usepackage{hhline}
\definecolor{lightyellow}{RGB}{250, 250, 180}
\definecolor{HLYELLOW}{RGB}{240, 127, 0}
\definecolor{hlyellow}{RGB}{240, 127, 0}
\sethlcolor{lightyellow}

%%%%%%%%%%%%%
% Algorithm stuff
%%%%%%%%%%%%%
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{pifont}
\usepackage{amsmath}
% clash with acmart
\let\Bbbk\relax
\renewcommand{\algorithmicforall}{\textbf{for each}}
% Various for each, for each in parallel, for each mod P...
\def\ForEach{\ForAll}
\algdef{SE}[FOREACHIN]{ForEachIn}{EndForEachIn}[2]{\algorithmicfor\ \textbf{each}\ #1\ \textbf{in}\ #2\ \textbf{do}}{\algorithmicend\ \algorithmicfor}%
\algdef{SE}[FOREACHP]{ForEachP}{EndForEachP}[1]{\algorithmicfor\ \textbf{each}\ #1\ \textbf{in parallel do}}{\algorithmicend\ \algorithmicfor}%
\algdef{SE}[FOREACHINP]{ForEachInP}{EndForEachInP}[2]{\algorithmicfor\ \textbf{each}\ #1\ \textbf{in}\ #2\ \textbf{in parallel do}}{\algorithmicend\ \algorithmicfor}%
\algdef{SE}[FORMOD]{ForMod}{EndForMod}[3]{\algorithmicfor\ #1\ \textbf{from}\ #2\ \textbf{to}\ #3\ \textbf{do}}{\algorithmicend\ \algorithmicfor}%
\algdef{SE}[FORMOD]{ForModS}{EndForModS}[4]{\algorithmicfor\ #1\ \textbf{from}\ #2\ \textbf{to}\ #3\ \textbf{step}\ #4\ \textbf{do}}{\algorithmicend\ \algorithmicfor}%
\algdef{SE}[FORMODP]{ForModPS}{EndForModPS}[3]{\algorithmicfor\ #1\ \textbf{from}\ #2\ \textbf{to}\ #3\ \textbf{in parallel do}}{\algorithmicend\ \algorithmicfor}%
\algdef{SE}[FORMODP]{ForModP}{EndForModP}[4]{\algorithmicfor\ #1\ \textbf{from}\ #2\ \textbf{to}\ #3\ \textbf{step} #4\ \textbf{in parallel do}}{\algorithmicend\ \algorithmicfor}%

% FIXME - make it configurable

\iftoggle{AlgsNoEnd} {
  \algtext*{EndFunction}% Remove "end while" text
  \algtext*{EndIf}% Remove "end if" text
  \algtext*{EndFor}% Remove "end if" text
  \algtext*{EndForEachIn}% Remove "end if" text
  \algtext*{EndForEachP}% Remove "end if" text
  \algtext*{EndForEachInP}% Remove "end if" text
  \algtext*{EndForModP}% Remove "end if" text
  \algtext*{EndForModPS}% Remove "end if" text
  \algtext*{EndForModS}% Remove "end if" text
}{}

\algdef{SE}[VARIABLES]{Variables}{EndVariables}{\algorithmicvariables}
  {\algorithmicend\ \algorithmicvariables}
  \algnewcommand{\algorithmicvariables}{\textbf{global}}
\algnewcommand{\LineComment}[1]{\State \(\triangleright\) #1}
% https://tex.stackexchange.com/questions/50908/algorithms-and-boolean-operator-casuing-undefined-control-sequence-error
\algnewcommand{\And}{\textbf{and}\xspace}


%%%%%%%%%%%%%
% Tikz nodes in the text
%%%%%%%%%%%%%
% https://tex.stackexchange.com/questions/7032/good-way-to-make-textcircled-numbers
\usepackage{tikz}
\usepackage{pifont}
\usetikzlibrary{shapes}
\DeclareRobustCommand*\circled[1]{\tikz[baseline=(char.base)]{
\node[shape=circle,fill=brown,draw=brown,inner sep=0pt] (char) {\textcolor{white}{\small\textbf{#1}}};}}
\DeclareRobustCommand*\circledColor[2]{\tikz[baseline=(char.base)]{
    \node[shape=circle,fill=#2,draw=#2,inner sep=1pt] (char) {\textcolor{white}{\small\textbf{#1}}};}}
\DeclareRobustCommand*\circledColorSmall[2]{\tikz[baseline=(char.base)]{
    \node[shape=circle,fill=#2,draw=#2,inner sep=0pt] (char) {\textcolor{white}{\footnotesize\textbf{#1}}};}}
\DeclareRobustCommand*\nodeColor[3]{%
  \tikz[baseline=(char.base)]{%
    \node[shape=#3,fill=#2,draw=#2,inner sep=0pt] (char) {\textcolor{white}{\small\textbf{#1}}};%
  }%
}
\DeclareRobustCommand*\nodeColorSmall[3]{%
  \tikz[baseline=(char.base)]{%
    \node[shape=#3,fill=#2,draw=#2,inner sep=0pt] (char) {\textcolor{white}{\footnotesize\textbf{#1}}};%
  }%
}
\DeclareRobustCommand*\circledColorX[1]{\tikz[baseline=(char.base)]{
    \node[shape=circle,fill=#1,draw=#1,inner sep=2pt] {}
  }
}

%%%%%%%%%%%%%%
% C++ listings
%%%%%%%%%%%%%%
\usepackage{listings}
\newfloat{codeblock}{H}{myc}
%\newcommand{\code}[1]{\figure{#1}}
\definecolor{darkblue}{rgb}{0,0,.6}
\definecolor{darkred}{rgb}{.6,0,0}
%\definecolor{darkgreen}{rgb}{0,.6,0}
\definecolor{darkgreen}{rgb}{0,.5,0}
\definecolor{red}{rgb}{.98,0,0}
\definecolor{gray}{rgb}{.6,.6,.6}
\definecolor{newgreen}{RGB}{169,209,142}
\definecolor{newpurple}{RGB}{237,134,254}
\definecolor{neworange}{RGB}{244,177,131}
\definecolor{newyellow}{RGB}{255,217,102}
\lstloadlanguages{C++}
% Settings for the lstlistings environment
\lstset{
	language=C++,                       % choose the language of the code
  basicstyle=\footnotesize\ttfamily\linespread{0.8},  % the size of the fonts that are used for the
	%basicstyle=\scriptsize,  % the size of the fonts that are used for the
	% code
	numbers=left,                       % where to put the line-numbers
	numberstyle=\tiny,                  % the size of the fonts that are used for the
	% line-numbers
	stepnumber=1,                       % the step between two line-numbers. If it's
	% 1 each line will be numbered
	numbersep=5pt,                      % how far the line-numbers are from the code
	%backgroundcolor=\color{gray},      % choose the background color. You must add
	% \usepackage{color}
	showspaces=false,                   % show spaces adding particular underscores
	showstringspaces=false,             % underline spaces within strings
	showtabs=false,                     % show tabs within strings adding particular
	% underscores
	keywordstyle=\bfseries\color{black},  % color of the keywords
	commentstyle=\color{darkgreen},     % color of the comments
	stringstyle=\color{darkred},        % color of strings
	captionpos=b,                       % sets the caption-position to top
	tabsize=2,                          % sets default tabsize to 2 spaces
	frame=tb,                       % adds a frame around the code
	breaklines=true,                    % sets automatic line breaking
	breakatwhitespace=false,            % sets if automatic breaks should only happen
	% at whitespace
	%escapechar=\%,                      % toggles between regular LaTeX and listing
	%belowskip=0.3cm,                    % vspace after listing
	morecomment=[s][\bfseries]{struct}{\ },
	morecomment=[s][\bfseries]{class}{\ },
	morecomment=[s][\bfseries]{public:}{\ },
	morecomment=[s][\bfseries]{public}{\ },
	morecomment=[s][\bfseries]{protected:}{\ },
	morecomment=[s][\bfseries]{private:}{\ },
	morecomment=[s][\bfseries\color{black}]{operator+}{\ },
	xleftmargin=0.1cm,
  literate={\%}{\%}{1},
	%xrightmargin=0.1cm,
  aboveskip=0pt,
  belowskip=0pt,
}


==> secs/discussion.tex <==

%\textbf{How does our work translate to our cloud platforms?}
%\todo{Discuss Azure, GCP}

\textbf{Collective algorithms variety.}

Another interesting research direction is the extension of FMI with more collective algorithms.
%
We currently provide one optimized algorithm per collective and channel type. Thanks to extensive research in this area, it is known that the best performing algorithm depends on various factors and different selection mechanisms have been developed.
%\cite{mamidalaMPICollectivesModern2008,liImprovedMPICollectives2014,pjesivac-grbovicPerformanceAnalysisMPI2007,hunoldAutotuningMPICollectives2018,mirsadeghiTopologyAwareRankReordering2016,hoeflerImplementationPerformanceAnalysis2007}.
FMI is well suited for the integration of additional collective algorithms and dynamic selection at runtime. Cost is an additional interesting design dimension, as the fastest collective algorithm may not be the cheapest.
Finally, the performance of collectives can be sensitive to imbalance and noise~\cite{faraj2008study,10.1145/3208040.3208054}
and require dynamic adaptive schemes for robustness~\cite{faraj2008study,4536308}.
%
This is a significant problem in serverless, where performance variability is high~\cite{copik2021sebs}.

\textbf{Dynamic group membership.}
Ephemeral functions can be used to implement adaptive and dynamic parallelism
of \emph{evolving} and \emph{malleable} applications~\cite{10.1007/BFb0022284}.
%
Thus, serverless group communicators could support joining and leaving the group by functions at any time.
While this topic is beyond the scope of this paper, it would bring the communication models closer to the serverless ecosystem and allow a more seamless integration.
